A tree-based kernel for graphs with continuous attributes

The availability of graph data with node attributes that can be either discrete or real-valued is constantly increasing. While existing kernel methods are effective techniques for dealing with graphs having discrete node labels, their adaptation to non-discrete or continuous node attributes has been limited, mainly for computational issues. Recently, a few kernels especially tailored for this domain, and that trade predictive performance for computational efficiency, have been proposed. In this paper, we propose a graph kernel for complex and continuous nodes' attributes, whose features are tree structures extracted from specific graph visits. The kernel manages to keep the same complexity of state-of-the-art kernels while implicitly using a larger feature space. We further present an approximated variant of the kernel which reduces its complexity significantly. Experimental results obtained on six real-world datasets show that the kernel is the best performing one on most of them. Moreover, in most cases the approximated version reaches comparable performances to current state-of-the-art kernels in terms of classification accuracy while greatly shortening the running times.

==> DDKernel_edge.tex <==
\section{Ordered Decomposition DAG Kernels for Graphs} \label{sec:oddkernel}

This section briefly recalls the ODD graph kernel framework~\cite{Dasan2012}. 
Let us first introduce some notation. A graph $G=(V,E,\labelfun)=(V_G,E_G,\labelfun)$ is a triplet where $V$ ($V_G)$ is the set of vertices, $E$ ($E_G$) the set of edges and $\labelfun()$ a function mapping nodes to labels. The number of vertices $|V|$ in a graph is usually referred as $n$, while the number of edges as $m$. A graph is undirected if $(\node_i,\node_j)\in E \Leftrightarrow (\node_j,\node_i)\in E$, otherwise it is directed. A path $\path(\node_i, \node_j)$ of length $n$ in a graph $G$ is a sequence of nodes $\node_1,\ldots,\node_n$, where $\node_1=\node_i$, $\node_n=\node_j$ and $(\node_k,\node_{k+1})\in E$ for $1\leq k< n$. A cycle is a path for which $\node_1=\node_n$. A graph is acyclic if it has no cycles. A tree is a directed acyclic graph where each node has at most one incoming edge. The root of a tree $T$ is represented by $r(T)$. A proper subtree rooted at node $\node$ comprises $\node$ and all its descendants.

The idea of the ODD kernel framework is to decompose the input graph into a set of substructures for which the test of isomorphism can be performed efficiently, i.e. subtrees. 
%The strategy for defining kernels that the framework employs is to decompose the input graph into a set of substructures for which the test of isomorphism can be performed efficiently, i.e. subtrees.


%This is ultimately obtained by mapping the input graphs into two sets of DAGs and then applying a kernel for DAGs on each pair of DAGs in the two sets. This kernel for DAGs consider subtrees as features.

 In order to map the graphs into trees, two intermediate steps are needed:
 %(see down in the section for further details). In the first one, the graph is decomposed into a multiset of unordered DAGs. The decomposition ensures that isomorphic graphs are represented by the same multisets of DAGs \cite{Dasan2012}. Since the vast majority of DAG kernels are extensions of ordered tree kernels, including the one we are going to use in the paper, an ordering between DAG nodes is defined. Finally, any Ordered DAG (ODD) is mapped into a multiset of trees by via the DAG kernel.




%The following scheme summarizes the steps for defining the kernel for graphs (see \cite{Dasan2012} for further details):  
\begin{enumerate}
 \item map the graph $G$ into a multiset of DAGs $\{DD_{G}^{\node_{i}} | \node_{i} \in V_{G} \}$, where $DD_{G}^{\node_{i}}$ is formed by the nodes and the edges in the shortest path(s) between $\node_i$ and any $\node_j\in V$. 
  %Fig.~\ref{fig:dagconstruction} gives an example of DAG decomposition of a graph. 
  It is possible to show that isomorphic graphs are represented exactly by the same multiset of DAGs $DD_{G}$. 
  %Since the visit is repeated for every node in $G$, any edge, which is not a self-loop, appears at least in one $DD_{G}^{\node_{i}}$. 
%   The Decomposition DAGs kernel for graphs can be defined as $DDK_{K_{DAG}}(G_1,G_2) = \displaystyle \sum_{D_1 \in DD(G_1)} \sum_{D_2 \in DD(G_2)} K_{DAG}(D_1,D_2).$
  %\begin{equation}
 % $DDK_{K_{DAG}}(G_1,G_2) = \displaystyle \sum_{\substack{D_1 \in DD(G_1) \\D_2 \in DD(G_2)}} K_{DAG}(D_1,D_2).$
  %\label{eq:dagk}\end{equation} 
  %The kernel of eq.~\eqref{eq:dagk} is an instance of the Haussler convolution kernel framework \cite{Haussler1999} and thus it is positive semidefinite for any positive semidefinite kernel $K_{DAG}$. 
  \item Since a vast class of DAG kernels can be easily derived from the extension of a kernel for ordered trees 
 % Since the kernel we are going to introduce requires the nodes to be ordered and $DD_{G}^{\node_{i}}$ ones are not,
   a strict partial order between DAG nodes in $DD_{G}^{\node_{i}}$ is defined yielding the Ordered Decomposition DAGs $ODD_{G}^{\node_{i}}$ as follows. 
   Let $\kappa()$ be a perfect hash function and $\#,\lceil,\rfloor$ be symbols never appearing in any node label, then 
   $\hash(\node)=L(\node)$ if $\node$ is a leaf node and $\hash(\node)=\kappa\big(L(\node)\big\lceil \hash(ch_\node[1])\#\hash(ch_\node[2])\ldots\#\hash(ch_\node[\rho(\node)])\big\rfloor\big)$ otherwise. 
  Now, the nodes of $DD_{G}^{\node_{i}}$ can be efficiently sorted according to $\hash(\node)$ values. Such ordering ensures that the swapping of non comparable nodes does not change the feature space representation of the examples \cite{Dasan2012}. %, i.e. the map
   % A more efficient ordering will be defined in Section~\ref{sec:hm}. 
 \item Finally, any Ordered DAG (ODD) is mapped into a multiset of trees. 
 Let us define $T(\node_i)$ as the tree resulting from the visit of $ODD_{G}^{\node_{i}}$ starting from node $\node_i$: the visit returns 
 the nodes reachable from $\node_{i}$ in $ODD_{G}^{\node_{i}}$. 
 If a node $\node_{j}$ can be reached more than once, more occurrences of $\node_{j}$ will appear in $T(\node_{i})$.  
 In the following, the notation $T_j(\node_i)$ indicates a tree visit of depth $j$. 
 %Fig.~\ref{fig:treevisits} gives an example of tree visits of two DAGs.
  %Notice that any node $\node_j$ of the DAG having $l>1$ incoming edges will be duplicated $l$ times in $T(\node_i)$ (together with all the nodes that are reached from $\node_j$ in the same visit). 
%  Now it is possible to extend any of the tree kernels defined in Section~\ref{sec:kernelsfortrees} to ordered DAGs:
  %Now the set $ODD_{G}$ has been transformed into a multiset of trees and thus, the kernel of eq.~\eqref{eq:st} can be applied as
 % \begin{equation}
 %  \label{eq:dagkernel}
%$	K_{ODAG}(OD_1,OD_2)=\sum_{\substack{\node_1\in V_{OD_1}\\\node_2\in V_{OD_2}}}C(r(T(\node_1)),r(T(\node_2))), $
 %  \end{equation}
 %  where $C$ is any instantiation of Eq.~\ref{eq:csst}.
%   Notice that the tree visit $T(\node_i)$ can be stopped when the tree $T(\node_i)$ reaches a maximum depth $h$. Such tree is referred to as $T_h(\node_i)$. 
  %In order to control the computational complexity and add expressiveness to the kernel, all the contribution for every $T_j(\node_i)$,  with $1\leq j \leq h$ can be summed:
%   \begin{equation}
%     \label{eq:dagstkernel}
% 	K_{DAG}(D_1,D_2)=\sum_{\substack{\node_1\in V_{D_1}\\\node_2\in V_{D_2}}}\sum_{j=1}^h C(r(T_j(\node_1)),r(T_j(\node_2))).  
%    \end{equation} 
 % Finally, a kernel between graphs which uses the DAG decomposition shown in this section and the 
\end{enumerate}
 In \cite{Dasan2012} the Ordered Decomposition DAGs kernel is finally defined as
  % instantiated with the Subtree Kernel for trees 
   as:
  \begin{equation}
  \begin{array}{ll}
   K_{ODD}(G_1,G_2) = & \!\!\!\!\!\!\!\!\!\!\!\!\displaystyle \sum_{\substack{OD_1 \in ODD(G_1) \\OD_2 \in ODD(G_2)}} \sum_{\substack{\node_1\in V_{OD_1}\\\node_2\in V_{OD_2}}} \cdot \\ & \cdot \sum_{j=1}^h C(r(T_j(\node_1)),r(T_j(\node_2)))
  \end{array}
% 
%     K_{ODD}(G_1,G_2) = \!\!\!\!\!\!\!\!\!\!\!\!\displaystyle \sum_{\substack{OD_1 \in ODD(G_1) \\OD_2 \in ODD(G_2)}} \sum_{\substack{\node_1\in V_{OD_1}\\\node_2\in V_{OD_2}}}\!\sum_{j=1}^h C(r(T_j(\node_1)),r(T_j(\node_2)))
    \label{eq:k}
  \end{equation}
 % The kernel of eq.~\eqref{eq:k} is the one which is used in the remainder of the paper. 
where $C()$ is a function defining a tree kernel. 
Among the kernels for trees defined in literature, the one employed in the paper is the Subtree Kernel (ST) \cite{DBLP:conf/nips/ViswanathanS02}, 
which counts the number of shared proper subtrees between the two input trees and have complexity $O(|V_T| \log |V_T|)$. 
We recall that the tree visits can be limited to a depth $h$ and that, consequently, the size of the tree visits is constant if we assume $\rho$ constant. 
In \cite{Dasan2012} it is shown that the ODD kernel with ST as tree kernel has complexity $O(|V_G|\log |V_G|)$. 
Other examples of popular tree kernels that can be used in the ODD framework are \cite{Collins2001} and \cite{Moschitti2006a}, which have associated a set of feature richer than the ST one. However, their computational complexity increasing leading to a $O(|V_T|^2 \log |V_T|)$ complexity for the ODD kernel (if we consider $\rho$ constant). 

% Another kernel worth citing is the Partial Tree kernel \cite{Moschitti2006a}, that considers all the possible subtrees of the given trees. Its complexity is $O(\rho^3 |V_T|^2)$, where $\rho$ is the maximum out-degree of the two trees, while the complexity of the associated graph kernel is $O(|V_T|^2 \log |V_T|)$, if we consider $\rho$ constant.
% \begin{figure}
% \centering
% \begin{tikzpicture}[auto,thick,scale=.5]
%    \tikzstyle{node}=[minimum size=12pt, inner sep=0pt, outer sep=0pt,ball color=blue,circle, text=white]
%   \small
% 	 \draw [red,->,line width=5pt] (-14.8,-1.5)--(-12.6,-1.5);
%  	 \draw [red,->,line width=5pt] (-14.8,-6.0)--(-12.6,-6.0);
%     \node [node, xshift=-8.4cm] {\textbf{s}} [->] %[->, ultra thick]
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (d2)[node, xshift=0.35cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b2) [node]{\textbf{e}}[]
%                 }
% 				;
%          \draw [->]
%          (b2) to (d2)
%         ;
%  	 \node [yshift=-0.8cm, xshift=-9.3cm] {a)};
%        \node [node, xshift=-8.4cm, yshift=-2.3cm] {\textbf{s}} [->] %[->, ultra thick]
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b2) [node]{\textbf{e}}[]
%                     child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
% 				;
%         ;     
%      	 \node [yshift=-3.1cm, xshift=-9.3cm] {b)};  
%      	    \node [node, xshift=-5cm] {\textbf{s}} [->] %[->, ultra thick]
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b2) [node]{\textbf{e}}[]
%                     child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
% 				;
%         ;
%            \node [node, xshift=-3.8cm] {\textbf{e}} [->]
%            child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
%            \node [node, xshift=-3.0cm] {\textbf{b}} [->]
%            child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
%            \node [node, xshift=-2.2cm] {\textbf{d}};          
%      	 %\node [yshift=-3.1cm, xshift=-5.0cm] {b)};  
%      	    \node [node, xshift=-5cm, yshift=-2.3cm] {\textbf{s}} [->] %[->, ultra thick]
%                 child {
%                     node [node] {\textbf{b}}[] 
%                     child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
%                 child {
%                     node (b2) [node]{\textbf{e}}[]
%                     child {node (d3)[node, xshift=0.0cm]{\textbf{d}}[]}
%                 }
% 				;
%         ;
%            \node [node, xshift=-3.8cm, yshift=-2.3cm] {\textbf{e}} [->]
%            child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
%            \node [node, xshift=-3.0cm, yshift=-2.3cm] {\textbf{b}} [->]
%            child {node (d2)[node, xshift=0.0cm]{\textbf{d}}[]};
%            \node [node, xshift=-2.2cm, yshift=-2.3cm] {\textbf{d}};
%            \node [node, xshift=-1.4cm, yshift=-2.3cm] {\textbf{d}};          
% \end{tikzpicture}
% \caption{TODO rimuovere ? Two DAGs (left) and their associated tree visits $T()$ starting from each node.\label{fig:treevisits}}
% \end{figure}

\section{A Graph Kernel for Continuous Node Labels and Edges} \label{sec:stcontinuous}

% In many real world problems, node and edge labels may belong to complex domains, such as real numbers and vectorial data \cite{bl}. 
% Kernels for discrete data tend to perform poorly when node labels belong to continuous domains due to sparsity issues \cite{bl}. 
This section shows a class of novel kernels for graphs able to deal with edge labels and non-discrete node labels. 
Our strategy is to extend some the tree kernels to complex node and edge labels. 
We focus on the ST kernel in the following, but similar changes can be easily applied to other kernels. 
First a few definitions need to be extended to the continuous domain. 
Let $L()$ be a labeling function that maps nodes to a generic codomain $\cal{X}_L$. 
Similarly, a function $L_E()$, whose codomain is $\cal{X}_E$, returns the label of a specific edge. 
Let us assume a total ordering for $\cal{X}_L$ and $\cal{X}_E$ is defined. 
The ordering described in section~\ref{sec:oddkernel} can be extended to include other values, such as edge labels, by prepending the representation of the edge to the one of the corresponding child node: 
$\pi(v)=\kappa\big(L(\node)\big\lceil \hash{(\node,ch_\node[1])}\#\hash(ch_\node[1])\#\ldots$ $\ldots\#\hash{(\node,ch_\node[\rho(\node)])}\#\hash(ch_\node[\rho(\node)])\big\rfloor\big) $. 
In addition, when dealing with complex node labels composed by pairs $(x_1, x_2)$ where $x_1$ is a ``standard'' discrete label and $x_2$ a vector of size $d$ of real values, if the $\pi()$ function returns the same value for two nodes, an additional function $\pi'(x_2)$ can be used for the (stable) ordering of $x_2$ values.
In our experiments, the $\pi'(x_2)$ function has been defined as the norm of the vector $x_2$.
% In addition, when the $\pi(v)$ values are the same, we can sort according to $\big\lceil\pi'(v)\big\rfloorthe$ formula takes into account complex node labels composed by pairs $(x_1, x_2)$ where $x_1$ is a ``standard'' discrete label and $x_2$ a vector of size $d$ of real values, by using an additional function $\pi'()$ for ordering $x_2$ values.
Such setting is the one of our experimental section. Such ordering does not exclude that two sibling, differing only in the vectorial labels of their children, can have the same $\pi()$ and $\pi'()$ values, but this will will not change the mapping in feature space of the examples because the kernel consider only the information extracted by the $\pi()$ and $\pi'()$ functions.Thus, the particular ordering of two sibling nodes with the same $\pi()$ and $\pi'()$ function values is ininfluent, i.e. the kernel function will be well defined. 
% 
% However, in the experimental section
% As an example, in the experimental section $\cal{X}_L$ is composed by pairs $(x_1, x_2)$ where $x_1$ is a ``standard'' discrete label and $x_2$ a vector of size $d$ of real values. 
% The ordering we employ first compare alphabetically $x_1$ values, only if two nodes are equivalent their corresponding $x_2$ values are compared. 
% 
% In order to clarify 
% 
% 
% TODO The order have to be extended to consider the vectorial labels. If two nodes that need to be ordered (siblings) have the same $\big(L(\node)$ value, the kernel value between each node and the (common) parent is considered for the ordering. If this value is the same, than a simple ordering between the vectors of the sibling nodes is used. 
% Note that if two sibling 

% Note that all the results in Section~\ref{} do not depend on the . 
%Let us assume a kernel for labels, $K_L:\cal{X}_L\times\cal{X}_L$, and a kernel for edges, $K_E:\cal{X}_E\times\cal{X}_E$ are available. 
In order to instantiate to the kernel employed in our experiments, we define a kernel on discrete node labels $K_{LD}(\node_1, \node_2)=\lambda$ (a kernel parameter) if $\node_1$ and $\node_2$ have identical discrete labels, $0$ otherwise. We further assume a kernel on vectorial labels $K_{LV}(\node_1, \node_2)$ and a kernel for edges $K_E((v_1,v_2),(v_3,v_4))$. 
Let us first extend the $C()$ function of ST defined in \cite{Collins2001} to handle edge labels: $C_{ST}(\node_1, \node_2) = K_{LD}(\node_1, \node_2)$ if $\node_1$ and $\node_2$ are leaves, and 
\begin{equation}
\begin{array}{ll}
 C_{ST}(\node_1, \node_2) = & K_{LD}(\node_1, \node_2) \\ & \cdot \prod_{j=1}^{nc(\node_1)} K_E((\node_1, ch_j[\node_1]), (\node_2, ch_j[\node_2]))\\ & \cdot C_{ST}(ch_j[\node_1]  ch_j[\node_2])
\end{array}
 \label{eq:cste}
\end{equation}
if $\node_1$ and $\node_2$ have the same number of children, $0$ otherwise. 

Then, the way we chose to extend the $C()$ function of ST defined in \cite{Collins2001} to handle complex node labels and edges is the following: 
\textit{i}) if $\node_1$ or $\node_2$ are leaf nodes then $C_{CST}(\node_1,\node_2)=K_{LD}(\labelfun(\node_1),\labelfun(\node_2))K_{LV}(\labelfun(\node_1),\labelfun(\node_2))$;\\
\textit{ii}) if $\node_1$ and $\node_2$ are not leaf nodes and $\rho(\node_1)=\rho(\node_2)$ then
	\begin{equation}
	  \begin{array}{l}
	    \displaystyle C_{CST}(\node_1,\node_2)=K_{LV}(\labelfun(\node_1),\labelfun(\node_2))C_{ST}(\node_1, \node_2), 
	  \end{array}
	  \label{eq:cst}
        \end{equation}
Note that the kernel for complex node labels is applied only to the root nodes of the tree. However, if $C_{CST}(\node_1,\node_2)>0$ then $C_{CST}(\node_1',\node_2')>0$ for any $\node_1'$ descendant of $\node_1$ and $\node_2'$ descendant of $\node_2$. As a consequence, the kernel $K_{LV}()$ is evaluated on all the descendants of $\node_1$ and $\node_2$. 
The kernel in eq.~\eqref{eq:k}, instantiated with the tree kernel in eq.~\eqref{eq:cst}, is positive semidefinite kernel since it is a finite product of positive semidefinite kernels, and the ordering function adopted for the children ordering is well-defined. We call it ODDCL$_{ST}$ kernel.  

Eq.\eqref{eq:cst} has the only the purpose to show how the computation of the ST kernel changes from the discrete to the complex node label domain. 
The algorithm we are going to use to compute the kernel is shown in the following section.  
%Assuming the complexity of $K_L()$ and $K_E()$ are  
% Following the reasoning at the end of Section~\ref{sec:treekernelsfordags}, the complexity of the kernel in \eqref{eq:ccsst} is $O(n^2H^2 Q(K_E) Q(K_L))$, where $Q(K_E)$ and $Q(K_L)$ are the worst case complexities of the kernels $K_L()$ and $K_E()$. 




==> IEEEtran/README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************

